Efficient Online Learning of Optimal Rankings: Dimensionality Reduction via Gradient Descent

We consider a natural model of online preference aggregation, where sets of preferred items $R_1, R_2, \ldots, R_t$ along with a demand for $k_t$ items in each $R_t$, appear online. Without prior knowledge of $(R_t, k_t)$, the learner maintains a ranking $\pi_t$ aiming that at least $k_t$ items from $R_t$ appear high in $\pi_t$. This is a fundamental problem in preference aggregation with applications to, e.g., ordering product or news items in web pages based on user scrolling and click patterns. The widely studied Generalized Min-Sum-Set-Cover (GMSSC) problem serves as a formal model for the setting above. GMSSC is NP-hard and the standard application of no-regret online learning algorithms is computationally inefficient, because they operate in the space of rankings. In this work, we show how to achieve low regret for GMSSC in polynomial-time. We employ dimensionality reduction from rankings to the space of doubly stochastic matrices, where we apply Online Gradient Descent. A key step is to show how subgradients can be computed efficiently, by solving the dual of a configuration LP. Using oblivious deterministic and randomized rounding schemes, we map doubly stochastic matrices back to rankings with a small loss in the GMSSC objective.

==> secs/intro.tex <==
Testing some notes.
\dimi{Testing.} \dimitodo{Side note by adding todo. Commands dimitodo, thanatodo, geotodo, stratitodo.}
\thana{Testing.}
\geo{Testing.}
\strati{Testing.}


A numerous number of practical applications involves presenting a set of items to users that sequentially arrive \cite{CKMS01,FSR18,GP13}. The order according to which the items are presented may result in vast differences in the overall performance of the system. Typically the later the items that interest a user appear in the order, the worse the performance of the system is for this specific user.  For example consider an online-store selling shoes. The web-designer must decide the top-down order of the available shoes such as each user finds shoes that interest her as high as possible. Obviously different orderings of the shoes may substantially affect the sales of the store since users with preferences appearing in the lower positions of the ordering admit less chances of performing a buy. %The latter 
Such phenomena may appear in various contexts. For example a study in the review process of 
$42$ computer science conferences revealed that early-submitted papers received greater number of bids because the papers were presented to the reviewers according to the submission ID number \cite{GP13}.

This kind of settings are typically modelled by the so-called \emph{Generalized Min-Sum Set Cover problem} (\gms) that has been extensively studied in the operational research literature.
In \gms, %\emph{ generalized min-sum set cover problem}, 
we are given a universe of items $U=\{1,\ldots,n\}$ and a sequence of requests $R_1,\ldots R_T \subseteq U$. 
Each request $R \subseteq U$ is associated with a covering requirement $\mathrm{K}(R) \leq |R|$. The goal is to find the permutation of the element $\pi^\ast \in [n!]$ minimizing the overall \textit{access cost}, $\pi^\ast = \argmin_{\pi \in [n!]}\sum_{t=1}^T \acost(\pi,R_t)$ where
\begin{equation}\label{eq:access_cost}
\acost(\pi,R_t) = \{\text{the first index up to which } \mathrm{K}(R_t) \text{ elements of }R_t \text{ appear in } \pi\}.  
\end{equation}
\noindent The special case in which $\mathrm{K}(R)=1$ for all requests $R$, is called \emph{Min-Sum Set Cover problem} (\ms) and is the version of the problem that was originally studied by \cite{FLP04}%\footnote{\GP{Do we have an intuitive example where the first index that covers elements is our cost? I.e. Our cost is not just increasing with the index but it is the index. It seems that there is a natural story in terms of having to inspect a list serially up until you can serve the request and the cost is exactly the number of items you have to inspect.}
%}.

Due to its wide range applications, there has been an intense interest towards the design of efficient algorithms producing (approximately) optimal permutations for \gms{}  \cite{HA05,FLP04,BGK10,AGY09,AG11,BGK10,INZ12,IS12,SW11}. Unfortunately even for the special case of \ms{}, 
not only finding the optimal permutation is $\mathrm{NP}$-hard, but also a permutation with approximation ratio less than $4$ cannot be found in polynomial time, unless $\mathrm{P}=\mathrm{NP}$. On the positive side, a simple greedy algorithm produces a $4$-approximate solution for \ms{}  \cite{FLP04}. For \gms{} the $4$-inapproximability lower bound directly transfers from 
\gms{}, while the state-of-art approximation ratio is $12.5$ produced by a randomized algorithm \cite{IS12}. Closing the gap between $4$ and $12.5$ remains an open question.
 
\noindent \textbf{\emph{Generalized Min-Sum Set Cover and Online Learning.}} Combinatorial optimization literature (offline) frequenly assumes that data avaliable to the algorithm well in advance. In terms of \gms{}  this means that the arriving requests are known to the algorithm up-front. However in most practical settings such information is not avaliable up-front, but is revealed as the system runs. For example although it is very hard for an online-store to have reliable information on the shoe-preferences its future clients, this information can be easily acquired as the systems runs by monitoring the clicks of the users.

%it is very easy to gradually acquire such information as users visit the sOnce a user visited the online store, the web-designer
%can easily learn which subset of shoes interest her by her clicks, while this acquired information can be used to update the ordering. The goal of the web-designer is to develop a computationally efficient permutation-selecting strategy, that guarantees a payoff close to the payoff of the optimal permutation. 

Towards the above-presented direction we cast 
\gms{} as an \textit{online learning problem} \cite{H16}. In this setting, there is a $\textit{learner}$
selecting permutations over time trying to minimize her overall cost and an adversary selecting the requests $R_1,\ldots,R_T$ trying to maximize the learner's overall cost. More precisely, at each round $t \geq 1$,
\begin{enumerate}
    \item The learner selects a permutation $\pi_t$ of the $n$ items, i.e., $\pi_t \in [n!]$.
    
    \item The adversary selects a request $R_t$ with
    covering requirements $\mathrm{K}(R_t)$.
    
    \item The learner's cost is $\acost(\pi_t,R_t)$ of Equation~\ref{eq:access_cost}.
\end{enumerate}
\noindent The \textit{learner} seeks for an \textit{online learning algorithm} that based on the requests $R_1,\ldots,R_{t-1}$, selects the permutation
$\pi_t$ (possibly with the use of randomization) such that the overall (expected) cost that she suffers is approximately bounded by the overall cost of the optimal permutation $\pi^\ast$. If the cost of the online learning algorithm is at most $\alpha$ times the cost of the optimal permutation, the algorithm is said to be $\alpha$\textit{-regret} \cite{H16}, while if $\alpha = 1$ the algorithm is said to be 
\textit{no-regret}. This work sheds light on the following question,

\begin{question}\label{q:main}
Is there an online learning algorithm for \gms{} that $\textbf{i)}$ runs in polynomial time and $\textbf{ii)}$
is $\alpha$-regret for some small constant $\alpha$?
\end{question}

Despite the 
huge amount of work towards the design of online learning algorithms and the rich literature on (offline) approximation algorithms for \gms{}, Question~\ref{q:main} does not admit an easy answer.

Although the famous $\textit{Multiplicative Weights Update Algorithm } (\mathrm{MWU})$ developed for the
more general $\textit{Learning from Expert Advice}$ problem is a \textit{no-regret} for the online \gms{}, it heavily violates the polynomial-time requirement of Question~\ref{q:main}. Particularly $\mathrm{MWU}$ treats each different permutation as a different expert, meaning that it keeps and updates a weight vector of size $n!$. 
Unfortunately unless $\mathrm{P} = \mathrm{NP}$, 
this huge space and time inefficiency cannot be circumvented with more clever implementations of  $\mathrm{MWU}$ exploiting the specific structure of \gms{}. The reason is that, even for the special case of \ms{}, any $\alpha$-regret online learning algorithm  running in polynomial-time, cannot be converted to
an $\alpha$-approximation polynomial-time algorithm. But as \cite{FLP04} showed, such an $\alpha$-approximation polynomial-time algorithm
cannot exist for $\alpha <4$ unless 
$\mathrm{P} = \mathrm{NP}$.

At the same time, the offline approximation algorithms for \gms{} heavily rely on the knowledge of the overall request sequence and there is no clue on how these algorithms can be transformed to run in the online setting \cite{FLP04,AGY09,AG11,SW11,BGK10,IS12,INZ12}.
%These algorithms are separated in two major categories, the \textit{greedy algorithms} \cite{FLP04,AGY09,AG11} and the \textit{LP-based algorithms} \cite{SW11,BGK10,IS12,INZ12}. 
%In the first category the elements are ordered according to a greedy criterion e.g.\textit{ the number of requests that an element covers} meaning that such algorithms cannot be easily transformed to online learning algorithms since such global information in not available in the online learning setting. The second class of algorithms solves an adequate fractional linear program that serves as a lower bound on the optimal cost. Again, even \textit{writting} this linear program requires  knowledge of  all the requests $R_1,\ldots,R_T$.



\textbf{Our Approach and Techniques.} 
%Our technical contribution consists of 
Technically, for all our results, we perform in two major steps.

In the first step we provide a no-regret polynomial time algorithm   for an intermediate online learning problem in which the action space of the learner is the set of doubly stochastic matrices. In this intermediate online learning problem, since the action space of the learner is the set of doubly stochastic matrices, the learner needs to determine only $n^2$ values at each time step, as opposed to the $n!$ values needed to describe a probability distribution over permutations.
This huge \textit{dimensionality reduction} allows to design a no-regret online learning algorithm for the intermediate problem that is subsequently used to provide the constant regret algorithms for the original problem. 

In the second step, for each of our results, we provide a (different) time efficient online rounding scheme that at each round converts the doubly stochastic matrix into a probability distribution over the permutations. The basic algorithmic challenge is guaranteeing that the expected cost of the (random) permutation produced by such schemes is at most $\alpha$-times greater than the cost of the respective doubly stochastic matrix of the intermediate problem. Once such a bound is established, it directly translates to an $\alpha$-regret online learning algorithm with respect to the optimal permutation for the original problem. Our  approach is summarized in Figure \ref{fig:general_scheme}.

\begin{figure}
    \centering
    \includegraphics{perm_14cm.png}
    \caption{The adopted general approach independent of the  variant of \gms{}}
    \label{fig:general_scheme}
\end{figure}
\textbf{Designing and Solving the Intermediate problem.} 
Examining an intermediate online learning problem with the set of doubly stochastic matrices as its action space,  comes as a natural relaxation of the original \gms{} problem. This is because any permutation of the elements can be encoded as an \textit{integral} doubly stochastic matrix where
each $0$-$1$ entry indicates whether a specific element lies in a specific position. In the intermediate problem, the request $R_t$ that the adversary selects at each round, associates each \textit{fractional doubly stochastic matrix} with a \textit{fractional accessing cost} that for \textit{integral doubly stochastic matrices} coincides with the \textit{original accessing cost} of \gms{}.

As already mentioned, at each round we convert the doubly stochastic matrix (produced for the intermediate problem)
to a probability distribution over the permutations. We perform this \textit{convertion step} in polynomial-time, while we guarantee that the \textit{expected access cost}
of the produced probability distribution is approximately bounded by the \textit{fractional access cost} of the doubly stochastic matrix. The latter must be seriously taken into account when \textit{designing} the fractional accessing cost since for most extensions of the \gms{}'s access cost to doubly stochastic matrices such guarantees cannot be established.

We select the \textit{fractional accessing cost} to be given by the value of a linear program with exponentially many constraints that involve the request $R_t$ and the selected doubly stochastic matrix. Since \textit{fractional accessing cost} is a convex function on the convex domain of doubly stochastic matrices, \textit{Online Projected Gradient Descent (OPGD)} \cite{Z03} can be used to obtain a no-regret online learning algorithm for the intermediate problem. However computing the subgradient-vectors in polynomial-time is far from being trivial due to the exponential size of the linear program describing the fractional access cost.
One of our main technical contribution consists in showing that subgradients can in fact be computed in polynomial-time via solving the dual of the linear program describing the fractional access cost.

\textbf{Our Results.} We provide several positive answers for Question~\ref{q:main}. We first design a $28$-regret online learning algorithm for  \gms{} that runs in polynomial time. For the important special case of  
\ms{} (where all requests have $\mathrm{K} (R_t) = 1$), we provide a polynomial-time online learning algorithm with regret $10.8638$, thus getting closer to the lower bound of $4$-regret of any polynomial-time online learning algorithm. Finally for  \ms{} problem, we present a \textit{deterministic} polynomial-time online-learning algorithm achieving regret $2 \max_{t}|R_t|$. The latter is surprising as it is a no-trivial upper bound on the regret of a learner that \textit{does not use randomization in her actions}.
Typically, learners that deterministically select their actions can achieve only trivial upper bounds on the regret. Recall that in the \textit{Learning From Expert Advice problem} any deterministic online learning algorithm cannot achieve regret better than $\Omega(\# \text{experts})$. The latter is equivalent to saying that  there
is no online learning algorithm (even randomized) achieving regret better than $\Omega(\# \text{expert})$ against a more \textit{powerful adversary that can see
the realization of the action of the learner before selecting the cost of each action}. Our last result reveals that in case of \ms{} a non-trivial regret bound of $2 \max_{t}|R_t|$ can be established against such powerful adversaries. Although $2 \max_{t}|R_t|$ can be arbitrarily larger than $10.86$ usually the size of the requests that arrive will be bounded ( e.g. the set of shoes interesting a potential buyer cannot be very large). Finally the above result is approximately tight since any deterministic online learning algorithm must have regret at least $\max_{t} |R_t|/2$. The state of the art and our results (in bold) are summarized below.

\begin{center}
 \begin{tabular}{||c c c c||} 
 \hline
 & Running Time & Upper Bound (Regret) & Lower Bound (Regret) \\ [0.5ex]
 \hline\hline
 \textit{GMSSC}&
% Generalized Min-Sum Set Cover} & 
Exponential ($\mathrm{MWU}$) & 1 & 1 \\
 \hline
 \textit{GMSSC}&%Generalized Min-Sum Set Cover} &
 Polynomial & $\boldsymbol{28}$ & 12.5 (for polyn. running time) \\
 \hline
 \textit{MSSC}&%{Min-Sum Set Cover} & 
 Polynomial & $\boldsymbol{10.8}$ & 4 (for polyn. running time) \\
 \hline
 \textit{MSSC}&%{Min-Sum Set Cover} & 
 Polyn. (deterministic) & $ \boldsymbol{2\cdot \max_{t}|R_t|}$ & $\max_{t}|R_t|$ (for any deterministic) \\
 \hline
 %5 & 88 & 788 & 6344 \\ [1ex] 
\end{tabular}
\end{center}



\textbf{Related Work.}
Our work relates with a long line of research concerning
the design of computationally efficient online learning algorithms in combinatorial domains. Such domains may include paths of a graph \cite{HS97}, permutations \cite{TW00,TM03} or even binary search trees. As already explained in such settings the vanilla $\mathrm{MWU}$ is no longer an option due to the exponential number of actions of the learner. As a result, this line of research developed algorithms by taking into account the combinatorial structure of each specific setting, and managed to mimic the distribution of $\mathrm{MWU}$ but with efficient implicit calculations.

Although the combinatorial domain in the forementioned online learning problems was completely different, all of the above settings shared the following common ground: \textit{the underlying combinatorial optimization problem is  easy.}
In their seminal work, \cite{KV03} unified all these ad-hoc approaches by showing
that any polynomial-time algorithm producing an optimal solution for the underlying combinatorial optimization problem, can be converted into 
a polynomial-time no-regret online learning algorithm.
Follow-up works \cite{RW17,S12,KWK10} improved the result
of \cite{KV03} for specific settings in which the underlying combinatorial optimization problem could be optimally solved by a specific algorithmic technique such as dynamic programming.  

All the forementioned line of research can be summarized in the following sentence, \textit{whenever the offline combinatorial optimization can be solved in polynomial time, there exists a no-regret online learning algorithm running in polynomial-time.}
One would expect that an approximate version of the above statement carries over in case the underlying combinatorial optimization problem is $\mathrm{NP}$-hard. More precisely, given an $\alpha$-approximation algorithm for the offline learning problem running in polynomial-time, one could design a polynomial-time $\alpha$-regret online learning algorithm for the online version of the problem. Unfortunately as \cite{KKL07} showed, this is not true. They presented an example in which the reduction of \cite{KKL07} fails to produce an $\alpha$-regret online learning algorithm, given an $\alpha$-approximation algorithm. On the positive side, 
\cite{KKL07} presented another algorithmic black-box reduction that converts any $\alpha$-approximation algorithm to an $\alpha$-regret algorithm. Their reduction is far more involved than the respective reduction of \cite{KV03} and only holds for a specific 
but fairly wide class of optimization problems called \textit{linear optimization problems}.

Last, there is a recent line of research \cite{YHKSTT11,A14,HW07} studying no-regret algorithms running in polynomial time for online learning problems concerning the selection of permutations. In
\cite{YHKSTT11,A14,HW07} is considered the setting where, once the the adversary reveals the request $R_t$, the learner pays the sum of the positions of $R_t$'s elements in permutation $\pi_t$. The basic difference of this setting with ours is that the underlying combinatorial optimization problem can be solved in polynomial-time, meaning that even the black-box reduction of \cite{KV03} produces polynomial-time online learning algorithms for this problem. As a result,  \cite{YHKSTT11,A14,HW07} focus on the design of polynomial-time no-regret algorithms that optimize the vanishing rate of the time-average regret.


==> secs/roundings.tex <==
Next, we present polynomial-time rounding schemes that map a doubly stochastic matrix back to a probability distribution on permutations. Our schemes ensure that the resulting permutation (random or deterministic) has access cost ~\eqref{eq:access_cost} at most $\alpha$ times the fractional access cost of the corresponding doubly stochastic matrix. Combining such schemes with the Algorithm~\ref{alg:projected_gradient_descent}, we obtain polynomial-time $\alpha$-regret online learning algorithms for \gms{}. 

We start by presenting the rounding scheme that solves the most general case (\textit{GMSSC}) that is based on the randomized rounding algorithm of \cite{SW11}.
\stratitodo{Probably mention that this schemes rounds the fractional solution of a different LP that the one we use. We cannot use it because there is no way to polynomially compute the sugradients of this LP.}
\begin{algorithm}[H]
  \caption{Converting Doubly Stochastic Matrices to Probability Distributions over Permutations}\label{alg:sampling_GMSSC}
  \textbf{Input:} A doubly stochastic matrix $A \in \mathrm{DS}$.\\
  \textbf{Output:} A randomly selected permutation such that Theorem~\ref{t:GMMSC-rounding} holds.
  \begin{algorithmic}[1]
  \State Randomly pick $\alpha \in (0,1)$ with probability density function $f(\alpha) = 2\alpha$.
  \State Construct the matrix $(5.03/\alpha) \cdot A$.
  \For{ all elements $e = 1$ to $n$ }
  \For{ all positions $j = 1$ to $\left \lfloor{n/2}\right \rfloor$ }
    \State $B_{e,2j} \leftarrow B_{e,2j} + B_{e,j}$.
  \EndFor
  \EndFor
  \For{ all elements $e = 1$ to $n$ }
    \State  Pick $\alpha_e$ uniformly at random in $[0,1]$.
    \State  Find the effecive index $i_e^\alpha \leftarrow \argmax_{i} \{i: \sum_{j=1}^{i-1}B_{ej} < \alpha_e\}$.
  \EndFor
  \State Output the elements according to the order of $i_e$'s.
    \end{algorithmic}
\end{algorithm}



\begin{theorem}\label{t:GMMSC-rounding}
Let $\mathrm{P_A}$ denote the probability distribution over permutations that Algorithm~\ref{alg:sampling_GMSSC} produces given as input $A \in \mathrm{DS}$. For any request $R$,
\[\E_{\pi \sim \mathrm{P}_A}[\acost(\pi,R)] \leq 28(1+\eps) \cdot \mathrm{FAC}_{R}(A)\]
\noindent where $\eps>0$ is the parameter used in Definition~\ref{d:artificial_cost}.
\end{theorem}

We now exhibit how Algorithm~\ref{alg:projected_gradient_descent} and Algorithm~\ref{alg:sampling_GMSSC} can be combined to a $28$-regret, polynomial-time, online learning algorithm %that achieves  
for \textit{Generalized Min-Sum Set Cover}. The learner runs Algorithm~\ref{alg:projected_gradient_descent} \textit{in the background}, while at each round $t$ uses matrix $A^t$
to produce a probability distribution over permutations via Algorithm~\ref{alg:sampling_GMSSC}.
\smallskip
\begin{eqnarray*}
\frac{1}{T}\sum_{t=1}^T \E_{\pi_t \sim \mathrm{P}_{A^t}}[\acost(\pi_t,R_t)]
&\leq&
\frac{1}{T} \cdot \sum_{t=1}^T 28(1+\eps)\cdot \mathrm{FAC}_{R_t}(A^t)~~\text{(Theorem}~\ref{t:GMMSC-rounding})\\
&\leq&
\frac{28}{T}(1+\eps) \cdot  \min_{A \in \mathrm{DS}}
\sum_{t=1}^T \mathrm{FAC}_{R^t}(A) + O\left(\frac{n^6}{\epsilon\sqrt{T}}\right)~~\text{(Theorem}~\ref{t:no-regret_artificial_cost})\\
&\leq&
\frac{28}{T}(1+\eps) \cdot
\sum_{t=1}^T \mathrm{FAC}_{R^t}(A^{\pi^\ast}) + O\left(\frac{n^6}{\epsilon\sqrt{T}}\right)\\
&\leq&
\frac{28}{T}(1+\eps) \cdot 
\sum_{t=1}^T \acost(\pi^\ast,R^t) + O\left(\frac{n^6}{\epsilon \sqrt{T}}\right)~~(\text{Corollary}~\ref{c:1})
\end{eqnarray*}
\noindent where the first inequality follows from Theorem~\ref{t:GMMSC-rounding}, the second from the no-regret property described in Theorem~\ref{t:no-regret_artificial_cost} and the last
from Corollary~\ref{c:basic}.

In Section~\ref{sec:MSSC_random} we present a modification of the Algorithm~\ref{alg:sampling_GMSSC}, that for the special case of \textit{Min-Sum Set Cover}, all requests $R_t$ have covering requirement $\mathrm{K}(R_t) = 1$, admits the approximation guarantee of Theorem~\ref{t:MMSC_rounding}. 
As a result, Algorithm~\ref{alg:sampling_MSSC} combined with Algorithm~\ref{alg:projected_gradient_descent} to produce a $11.713$-regret algorithm for the $\textit{online Min-Sum Set Cover problem}$.

\begin{theorem}\label{t:MMSC-rounding}
Let $\mathrm{P_A}$ denote the probability distribution over permutations that Algorithm~\ref{alg:sampling_MSSC} produces given as input $A \in \mathrm{DS}$. For any request $R$ with covering requirement $\mathrm{K}(R)=1$,
\[\E_{\pi \sim \mathrm{P}_A}[\acost(\pi,R)] \leq 11.713(1+\eps) \cdot \mathrm{FAC}_{R}(A)\]
\noindent where $\eps>0$ is the parameter used in Definition~\ref{d:artificial_cost}.
\end{theorem}

Finally in Section~\ref{sec:MSSC_deterministic}, we thee deterministic rounding scheme (Algorithm~\ref{alg:drand}) that converts any doubly stochastic matrix to a deterministic permutation of the elements with approximation guarantee of Theorem~\ref{t:det-rounding}.

\begin{algorithm}[H]
  \caption{Converting Doubly Stochastic Matrices to Permutations}\label{alg:drand}
  \textbf{Input:} A doubly stochastic matrix $A \in \mathrm{DS}$, a parameter $r$ and a parameter $\alpha >0$.\\
  \textbf{Output:} A deterministic permutation $\pi \in [n!]$.
  \begin{algorithmic}[1]
  \State $\text{Rem} \leftarrow \{1,\ldots,n\}$
  
  \For{$k = 1$ to 
  $\left \lfloor{n/r}\right \rfloor$ }
  
    \State $\mathrm{R_k} \leftarrow$ the set of elements $\in \mathrm{Rem}$ of size $r$ that is  
    a $(1+\alpha)$-approximate solution of the problem, \[\min_{R \in [\mathrm{Rem}]^r}\sum_{i=1}^n\max\left(1-\sum_{j=1}^{i-1}\sum_{e \in R}A_{ej},0 \right)\]
    
  \State Put the elements of $\mathrm{R_k}$ in positions $(k-1)\cdot r + 1$ to $k\cdot r$.
  
  \State $\text{Rem} \leftarrow \text{Rem} / \mathrm{R_k}$
  
  \EndFor
  \State \textbf{return} $\pi$.
  \end{algorithmic}
\end{algorithm}

\begin{theorem}\label{t:det-rounding}
Let $\pi_A$ denotes the permutation produced by Algorithm~\ref{alg:drand} when the doubly stochastic matrix $A$ was given as input. 
Then for any request $R$ with $\mathrm{K}(R)=1$
and $|R| \leq r$,
\[\acost(\pi_A,R) \leq 2 (1+\eps)(1+\alpha) r \cdot \mathrm{FAC}_{R}(A)\]
\noindent where $\eps>0$ is the parameter used in Definition~\ref{d:artificial_cost}. Moreover
Step~$3$ of Algorithm~\ref{alg:drand} can be implemented in $\Theta(n^4r^3/\alpha^2)$ steps.
\end{theorem}

As previously Algorithm~\ref{alg:drand} together with Algorithm~\ref{alg:projected_gradient_descent} produce a deterministic $ O(\max_{t} |R_t|)$-regret algorithm for the \textit{Online Min-Sum Set Cover problem}. Due to lack of space, the (1+$\alpha$)-approximation algorithm running in $\Theta(n^4/\alpha^2)$ for Step~$3$ of Algorithm~\ref{alg:drand} is presented in Section~\ref{s:DP}.

%\begin{theorem}\label{t:lower_bound}
%For any deterministic online learning algorithm there exits a sequence of requests $R_1,\ldots,R_T$ with $\mathrm{K}(R_t) = 1$ such that 
%\[\sum_{t=1}^T\acost(\pi_t,R_t) \geq (\max_{1\geq t \leq t}|R_t| / 2) \cdot \min_{\pi \in [n!]}\sum_{t=1}^T\acost(\pi^\ast,R_t)\]
%where $\pi_1,\ldots,\pi^T$ is the sequence of permutations produced by the online learning algorithm.
%\end{theorem}

